Motif Caller: Sequence Reconstruction for Motif-Based DNA Storage

DNA data storage is rapidly emerging as a promising solution for long-term data archiving, largely due to its exceptional durability. However, the synthesis of DNA strands remains a significant bottleneck in terms of cost and speed. To address this, new methods have been developed that encode information by concatenating long data-carrying DNA sequences from pre-synthesized DNA subsequences - known as motifs - from a library. Reading back data from DNA storage relies on basecalling - the process of translating raw nanopore sequencing signals into DNA base sequences using machine learning models. These sequences are then decoded back into binary data. However, current basecalling approaches are not optimized for decoding motif-carrying DNA: they first predict individual bases from the raw signal and only afterward attempt to identify higher-level motifs. This two-step, motif-agnostic process is both imprecise and inefficient. In this paper we introduce Motif Caller, a machine learning model designed to directly detect entire motifs from raw nanopore signals, bypassing the need for intermediate basecalling. By targeting motifs directly, Motif Caller leverages richer signal features associated with each motif, resulting in significantly improved accuracy. This direct approach also enhances the efficiency of data retrieval in motif-based DNA storage systems.

==> section_texts/background.tex <==

DNA sequencing has experienced rapid advancement since the early days of Sanger sequencing \cite{deamer2016three}. Today, high-throughput technologies, such as Nanopore sequencers, are readily accessible, making sequencing more cost-effective \cite{ceze2019molecular, mardis2013next}. Nanopore sequencing involves threading a DNA strand through a Nanopore that has an electrical current running through it \cite{mikheyev2014first}. As the DNA strand passes through, it disrupts the current, generating a series of electrical signal deflections that correspond to the individual bases. This produces a unique fingerprint for each base sequence. Machine learning based algorithms are then used to convert the recorded signal trace into a sequence of DNA bases, in a process known as basecalling.

Initially, basecalling was done by models like Hidden Markov Models (HMMs), with Oxford Nanopore Technologies (ONT) offering a cloud-based solution called Metrichor \cite{goldman2013towards}. As Nanopore sequencing grew in popularity, ONT and open-source alternatives shifted to using neural network architectures, such as Recurrent Neural Networks (RNNs), to provide local basecalling with a higher base-level accuracy \cite{wick2019performance, bovza2017deepnano}. While ONT’s basecallers used a segmentation approach to identify single bases, models like Chiron \cite{teng2018chiron} (an open-source alternative) used an end-to-end approach using Connectionist Temporal Classification (CTC) loss in a Convolutional Recurrent Neural Network (CRNN) architecture, achieving comparable accuracy without a segmentation step. Currently, standard basecallers like Dorado and Guppy also use such an architecture.

With the advent of portable devices like ONT's MinION sequencer, Nanopore sequencing has gained widespread adoption, especially in the field of DNA storage. Nanopore sequencing is particularly advantageous in DNA data storage due to its ability to handle long reads, which are crucial for high recovery rates \cite{ceze2019molecular}.

In motif-based DNA storage, data retrieval hinges on accurately identifying motifs. The baseline method of Motif Search (described in Sec. \ref{baseline}) detects a small fraction of the motifs per read that are within an information block. The goal of this paper is to increase the percentage of motifs that are detected per read over an information block. Since the percentage of motifs detected will be a small amount compared to the total information stored in the block (owing to errors in synthesis and sequencing), the complete information will be recovered by combining motif predictions of a number of reads over the same information block. The number of reads that are required to recover all the information for a block is called the effective sequencing coverage. By identifying a higher percentage of motifs per read, we in turn, seek to minimize the effective sequencing coverage.



==> section_texts/motif_based_synthesis.tex <==
In motif-based DNA storage, information is coded over a set of motifs, which are short subsequences of DNA. These motifs are pre-synthesized and combined to create a single block of information within a single strand called an oligo. This concept is shown in Fig.~\ref{fig:dataset}, where the basic structure of an oligo resulting from motif-based synthesis is shown. 

One end of the oligo is attached to a solid support, and motifs are added one by one to the growing strand. Each motif is separated by a spacer ($S$) in order to distinguish the boundary between two motifs and use the bridge ($B_x$) to join two motifs together. The spacers attach to each other using the bridge, which connects the two sections of the spacers using their complementary sequences.



\subsection{Helixworks' Combinatorial Approach} \label{helixworks}

Helixworks have developed a combinatorial approach to motif-based DNA storage \cite{yan2023scaling, sokolovskii2024coding}. To scale the logical density of each symbol, instead of coding over individual motifs, information is coded over subsets of motifs from a predefined motif library. In this way, the amount of information per symbol can be scaled from $\log_2 {M}$ to $\log_2{M \choose k}$ bits, where $M$ is the size of the motif library and $k$ is the number of motifs per symbol. In the Helixworks pipeline \cite{yan2023scaling}, there are 2 address slots and 8 payload slots within each block, where each requires one synthesis cycle. Each payload slot consists of 1 of the 4 motifs that constitutes a single combinatorial symbol. There are therefore 8 information carrying (payload) motifs in total in each cycle. Our datasets described in Sec.~\ref{dataset} results from the experimental runs of this pipeline. 


\subsection{CatalogDNA's Combinatorial Approach} \label{catalogdna}

CatalogDNA's \cite{roquet2021dna} approach, introduces a novel method for combinatorial based motif storage that similarly increases the logical density of each symbol. They operate over a set of DNA fragments (components) that are designed and partitioned into a fixed number of disjoint sets (layers). The components are prefabricated and are analogous to the concept of motifs (described in Sec. \ref{motif_based_synthesis}. Longer DNA molecules (identifiers) are assembled from these components by ligating them together, where only one component from each layer is chosen, and the layers have a pre-defined fixed order. 
The components are designed to have a unique central region and two edge sequences that are common to all components within a layer. The central region allows for random access, as it acts a unique primer binding site for the targeted selection of identifiers. The edge sequences are single strand overhangs designed to facilitate ligation between components of adjacent layers.


% Two column figure needs to be on previous page
\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{Figures/motif_based_synthesis.png}
    \caption{Illustration of the typical block-like oligo structure in the motif-based DNA storage pipeline. Using the bridge ($B_x$), the spacers ($S$) of two motifs are concatenated using their complementary sequences. Motifs are added one by one, growing the sequence.}
    \label{fig:dataset}
\end{figure}

The resulting identifier space represents all potential identifiers derivable from the initial component library. The complexity of the space grows exponentially with the number of layers, mathematically expressed as $\prod_{i=1}^{N} M_i$, where $N$ represents the total number of layers and $M_i$ indicates the number of components in that layer. To manage this space, CatalogDNA uses an ordered tree structure (called a C-tree), where each tree level corresponds to a specific layer. The tree's architecture ensures a fixed branch ordering, with each branch representing a component. This structure allows for a systematic collection of identifiers through a post-order traversal, enabling the assignment of a unique rank to each identifier.


This ranking mechanism is used to encode information. By selectively assembling and pooling identifiers corresponding to specific bit positions, the method can encode binary information.
\begin{figure*}[!b]
    \centering
    \includegraphics[width=\textwidth]{Figures/callercomparison.png}
    \caption{Figure illustrating the difference in operation between the Motif Search and Motif Caller pipelines for sequence reconstruction. A motif-based oligo containing the symbols $M_1, M_2, M_4$ passes through the nanopore (a) and produces a trace of the bases in the squiggle (b). The signal is used to predict a base level sequence using basecalling (c). From this base level sequence, Motif Search (d) is used to obtain the final motif sequence prediction. The Motif caller (e) shorts the two-step reconstruction by predicting the motif sequence directly from the squiggle.}
    \label{fig:pipeline}
\end{figure*}
